A Combination Theorem for Geodesic Coarsely Convex Group Pairs

The first author and Oguni introduced a class of groups of non-positive curvature, called coarsely convex group. The recent success of the theory of groups which are hyperbolic relative to a collection of subgroups has motivated the study of other properties of groups from the relative perspective. In this article, we propose definitions for the notions of weakly semihyperbolic, semihyperbolic, and coarsely convex group pairs extending the corresponding notions in the non-relative case. The main result of this article is the following combination theorem. Let $\mathcal{A}_{wsh}$, $\mathcal{A}_{sh}$, and $\mathcal{A}_{gcc}$ denote the classes of group pairs that are weakly semihyperbolic, semihyperbolic, and geodesic coarsely convex respectively. Let $\mathcal A$ be one of the classes $\mathcal{A}_{wsh}$, $\mathcal{A}_{sh}$, and $\mathcal{A}_{gcc}$. Let $G$ be a group that splits as a finite graph of groups such that each vertex group $G_v$ is assigned a finite collection of subgroups $\mathcal{H}_v$, and each edge group $G_e$ is conjugate to a subgroup of some $H\in \mathcal{H}_v$ if $e$ is adjacent to $v$. Then there is a non-trivial finite collection of subgroups $\mathcal{H}$ of $G$ satisfying the following properties. If each $(G_v, \mathcal{H}_v)$ is in $\mathcal{A} $, then $(G,\mathcal{H})$ is in $\mathcal{A}$. The main results of the article are combination theorems generalizing results of Alonso and Bridson; and Fukaya and Matsuka.

==> 16-questions-graph-of-groups.tex <==
Let $G=G_1\ast_C G_2$  denote the amalgamated product determined by
$G_1\xleftarrow{\partial_1}C\xrightarrow{\partial_2}G_2$. 
Suppose, for $i=1,2$,  $G_i$ admits a finite $G_i$-simplicial
 complex which is a universal space for proper actions.  
If $C$ is finite, then $G$ is hyperbolic relative to $\{G_1,G_2\}$, 
thus $G$ satisfies the coarse Baum-Connes conjecture by \cref{thm:cBC-relhyp}.
%The following questions are thegeneralizations of this argument.

\begin{question}
\label{conj:cBC-amalgamation}
Let $G=G_1\ast_C G_2$  denote the amalgamated product determined by
$G_1\xleftarrow{\partial_1}C\xrightarrow{\partial_2}G_2$. 
Suppose, for $i=1,2$,  $G_i$ admits a finite $G_i$-simplicial
 complex which is a universal space for proper actions.  
If $C$ is undistorted in both $G_1$ and $G_2$, then, 
does $G$ satisfy the coarse Baum-Connes conjecture?
Do similar statements for HNN-extensions hold?
\end{question}

More general question is the following.

\begin{question}
\label{conj:cBC-graph-of-groups}
 Let $G$ be a group that splits as a finite graph of groups such that 
 each vertex group $G_v$ and edge group $G_e$ satisfy 
 the coarse Baum-Connes conjecture, and admit a finite 
 $G_v$ ($G_e$, respectively)-simplicial complex which is a universal space for proper
 actions. Suppose that edge groups are not distorted in vertex groups.
 Then does $G$ satisfy the coarse Baum-Connes conjecture? 
% Can we remove the assumption on non-distorted condition?
\end{question}

==> 20-Preliminaries.tex <==
%\subsection{Relative geometric actions}

Let $G$ be a group and $\mathcal{H}$ be a finite collection of subgroups, and $X$ a geodesic metric space with a $G$-action by isometries. 

\begin{definition}
 The $G$-action on $X$ is \emph{properly discontinuous relative to $\mathcal{H}$} if every  bounded open subset $U\subset X$ the set $\{g\in G\colon U\cap g.U \neq \emptyset\}$ is contained in the union of finitely many left cosets of finitely many conjugates of subgroups in $\mathcal{H}$. More specifically, there are sequences $k_1,\ldots, k_\ell$ and $g_1,\ldots ,g_\ell$ of elements of $G$ and a sequence $H_1,\ldots ,H_\ell$ of subgroups in $\mathcal{H}$  such that $\{g\in G\colon U\cap g.U\neq \emptyset\}$ is contained in $k_1 H_1^{g_1} \cup \cdots \cup k_\ell H_\ell^{g_\ell}$.
\end{definition}

%\tomo{
%There exists a finite subset $S\subset G$, 
%finite sequences $\{(k_i,g_i,H_i):i=1,\dots,l\}$ of elements of 
%\begin{align*}
% S\times S \times \mathcal{H}
%\end{align*}
%and a (possibly infinite) 
%sequence $\{(p_\lambda,q_\lambda,H_\lambda):\lambda\in \Lambda\}$ of elements of 
%\begin{align*}
% S \times \left(\bigcup \mathcal{H}\right)\times \mathcal{H}
%\end{align*}
%
%such that
%$\{g\in G\colon U\cap g.U\neq \emptyset\}$ is contained in the following
%\begin{align*}
% \bigcup_{i=1}^{l}k_iH^{g_i} \cup
% \bigcup_{\lambda \in \Lambda} p_\lambda H^{q_\lambda}_{\mu_\lambda}
%\end{align*}
%}

%\hrulefill

\begin{definition}[\tomo{an alternative definition on relative p.d. action}]
 We say that subset $U\subset X$ is 
 \emph{contained in a union of finitely many left 
 cosets in $G/\mathcal{H}$ relative to $\mathcal{H}$}, if
 there exist a finite subset $S\subset G$ and
 a (possibly infinite) 
 sequence $\{(k_\lambda,g_\lambda,H_\lambda)\}_{\lambda\in \Lambda}$ of elements of 
 \begin{align*}
 S \times \left(S\cup \bigcup \mathcal{H}\right)\times \mathcal{H}
 \end{align*}
 %
 such that
$U$ is contained in the following subset
 \begin{align*}
 \bigcup_{\lambda \in \Lambda} k_\lambda H^{g_\lambda}_\lambda
 \end{align*}

%This is equivalent to the following: 
 The $G$-action on $X$ is 
 \emph{properly discontinuous relative to $\mathcal{H}$} 
 if every bounded open subset $U\subset X$ 
 the set $\{g\in G: U\cap g.U\neq \emptyset\}$ is
 contained in a union of finitely many left 
 cosets in $G/\mathcal{H}$ relative to $\mathcal{H}$.
\end{definition}

\tomo{MEMO: Should we replace 
$S \times \left(S\cup \bigcup \mathcal{H}\right)\times \mathcal{H}$ by
$ \left(S\cup \bigcup \mathcal{H}\right) \times \left(S\cup \bigcup \mathcal{H}\right)\times \mathcal{H}$ ?}


\begin{definition}
\label{def:rel-geometric-action}
The $G$-action on $X$ is \emph{geometric relative \tomo{to}
$\mathcal{H}$} if it is properly discontinuous \redsout{with respect to}
\tomo{relative to}
$\mathcal{H}$, is cocompact, and for every $H\in \mathcal{H}$ the fixed
point set $X^H$ is non-empty.
\end{definition}

\begin{example}[Actions on coned-off Cayley graphs are not necessarily relatively geometric]
Consider the group $G=\Z\times\Z$ and the collection of subgroups
$\mathcal{H}=\{\Z\times 0, 0\times\Z \}$. In this case, the coned-off
Cayley graph $\hat\Gamma(G,\mathcal{H})$ has diameter four, and its
$G$-action is not properly discontinuous \redsout{with respect to}
\tomo{relative to} $\mathcal H$.
\end{example}

For a group pair $(G,\mathcal{H})$, we shall say that the collection of cone points of $\hat\Gamma(G,\mathcal{H})$ is \emph{locally finite} if every ball of finite radius in $\hat\Gamma(G,\mathcal{H})$ contains finitely many cone points. 

\begin{proposition}[Coned-off Cayley graphs with relatively geometric actions]
Let $G$ be a group, $\mathcal H$ be a finite collection of subgroups,
and $S$ a finite (relative) generating set of $G$ (with respect to
$\mathcal H$). The $G$-action on the coned-off Cayley graph
$\hat\Gamma(G,\mathcal{H},S)$ is geometric with respect to $\mathcal H$
if the set of cone points of $\hat\Gamma(G,\mathcal{H},S)$ is locally
finite.
\end{proposition}
\begin{proof}
We only need to verify that $G$-action on $\hat\Gamma(G,\mathcal{H})$ is properly discontinuous relative to $\mathcal{H}$. It is enough to consider a collection $U$ of edges for which the collection $V_0$ of all endpoints has finite diameter in $\hat\Gamma(G,\mathcal{H})$. Let $V$ be the collection of cone points which are at distance at most one from a vertex in $V_0$. The set $\{g\in G\mid U\cap gU\neq\emptyset\}$ is as subset of $\{g\in G\mid V\cap gV\neq \emptyset\}$. Since $U$ has finite diameter, $V$ has finite diameter as well, and then by hypothesis $V$ is finite. Each element of $V$ is a left coset in $G/\mathcal{H}$, say $V=\{g_1H_1,\ldots , g_nH_n\}$. In this case, $\{g\in G\mid V\cap gV\neq \emptyset\}$ is contained in $\bigcup_{H\in \mathcal{H}}\bigcup_{i,j} g_jg_i^{-1}H^{g_i}$.  
\end{proof}

We are not aware whether the converse of the above proposition holds. 

\begin{lemma}\label{lem:RelativeProperAction}
 If $G$ acts geometrically on $X$ relative to $\mathcal{H}$, then there is a bounded open subset $U$ such that $G.U=X$, and in particular   $\{g\in G\colon g.U\cap U\neq \emptyset\}$ 
\tomo{contained in a union of finitely many left 
 cosets in $G/\mathcal{H}$ relative to $\mathcal{H}$}.
%is contained in the union of finitely many left cosets in $G/\mathcal{H}$.   
\end{lemma}
\begin{proof}
 Since the $G$-action on $X$ is cocompact, 
 there exists a compact subset  $K$ of $X$ such that $G.K=X$.
 Since the action is properly discontinuous relative 
 to $\mathcal{H}$, for each $x\in K$ there is a bounded 
 open subset $U_x$ such that 
 $\{g\in G\colon U_x\cap g.U_x\neq\emptyset\}$ 
%is contained in the union of finitely many left cosets in $G/\mathcal{H}$. 
\tomo{contained in a union of finitely many left 
 cosets in $G/\mathcal{H}$ relative to $\mathcal{H}$}.
 By compactness, $K$ is contained in a  
 finite union $U=U_{x_1}\cup \cdots \cup U_{x_\ell}$. 
 Since each $U_{x_i}$ is bounded, $U$ is bounded.  
\end{proof}

\begin{proposition}\label{prop:geomAction}
Let $G$ be a group and $\mathcal{H}$ a finite collection of subgroups. If $G$ acts geometrically relative to $\mathcal{H}$ on a geodesic metric space $X$ then:
\begin{enumerate}
    \item $G$ is finitely generated relative to $\mathcal{H}$; and
    \item if $S$ is a finite relative generating set of $G$ with respect to $\mathcal{H}$, then there is a quasi-isometry between the coned-off Cayley graph $\hat\Gamma(G,\mathcal{H},S)$ and $X$. 
\end{enumerate}
\end{proposition}
\begin{proof}
Let $x\in X$ and let $U_r$ be an open ball of radius $r$ and center $x$ in $X$ satisfying the conclusion of Lemma~\ref{lem:RelativeProperAction}. Hence any ball $U_R$ of radius with $R> r$ and center $x$ satisfies $G. U_R =X$. Without loss of generality, assume that $r>1$.

%In particular, there is a finite subset $\{k_1H_1^{g_1}, \ldots , k_nH_n^{g_n}\}$ where $f_i,g_i\in G$ and $H_i\in \mathcal{H}$ and  such that $\{g\in G\colon U_{2r}\cap g.U_{2r}\neq\emptyset\}$ is contained in $T= k_1H_1^{g_1}\cup\cdots\cup k_nH_n^{g_n}$. Let $S=\{g_1,\ldots ,g_n, k_1, \ldots , k_n\}$. 

\tomo{In particular, there exist a finite subset $S\subset G$ and
 a 
 sequence $\{(k_\lambda,g_\lambda,H_\lambda)\}_{\lambda\in \Lambda}$ of elements of 
$S \times \left(S\cup \bigcup \mathcal{H}\right)\times \mathcal{H}$
% \begin{align*}
% S \times \left(S\cup \bigcup \mathcal{H}\right)\times \mathcal{H}
% \end{align*}
 %
 such that
 $\{g\in G\colon U_{2r}\cap g.U_{2r} \neq \emptyset\}$ is contained in 
% $\bigcup_{\lambda \in \Lambda} k_\lambda H^{g_\lambda}_\lambda$.
%the following subset
 \begin{align*}
  T=\bigcup_{\lambda \in \Lambda} k_\lambda H^{g_\lambda}_\lambda
 \end{align*}
}

We claim that $S$ is a finite relative generating set of 
$G$ with respect to $\mathcal{H}$.

Let $g\in G$. Now we mimic the proof of the \tomo{Schwarz-Milnor's} lemma. If $g.x=x$ then $g\in  T$ by definition. In particular, $g$ is a product of elements of $S$ and $\bigcup \mathcal H$; moreover, note that $\dist_{\hat\Gamma}(1,g) \leq 5$ if $g\in T$.  Otherwise, suppose $x\neq g.x$ and consider a geodesic $\gamma\colon [0,1]\to X$   between $x$ and $g.x$. Then there is a finite sequence of real numbers $t_0=0<t_1<\cdots<t_\ell=1$ and a sequence $1=f_0,f_1,\ldots , f_\ell=g$ of elements of $G$ such that $\dist_X(\gamma(t_i),\gamma(t_{i+1}))<r$ and $\gamma(t_i) \in f_i.U_r$. Note that we can assume that $\ell\leq \frac{2}{r}\dist_X(x,g.x) + 1$. In particular, $f_i.U_{2r}\cap f_{i+1}.U_{2r} \neq \emptyset$  and hence 
$f_i^{-1}f_{i+1}$ belongs to 
%$k_1H_1^{g_1}\cup\cdots \cup k_nH_n^{g_n}$. 
\tomo{$\bigcup_{\lambda \in \Lambda} k_\lambda H^{g_\lambda}_\lambda$}.
Since $f_0=1$  and $f_\ell=g$, it follows that $g$ is a product of elements in $S$ and $\bigcup \mathcal{H}$. 
Specifically, 
\tomo{$f_i^{-1}f_{i+1} = k_{\lambda_i}h_{i}^{g_{\lambda_i}}$} with
\tomo{$\lambda_i\in \Lambda$} and
$h_i\in \bigcup\mathcal{H}$. So we have  


%\[g= k_{j_1}g_{j_1}h_1g_{j_1}^{-1}  \cdots k_{j_{\ell-1}}g_{j_{\ell-1}}h_{\ell-1}g_{j_{\ell-1}}^{-1},\]

\[
 g= k_{\lambda_1}g_{\lambda_1}h_1g_{\lambda_1}^{-1}  
 \cdots k_{\lambda_{\ell-1}}g_{\lambda_{\ell-1}}h_{\ell-1}g_{\lambda_{\ell-1}}^{-1},
\]

 
which in $\hat\Gamma(G,\mathcal{H},S)$ describes a path of length $5(\ell-1)$ from $1$ to $g$. 

\tomo{MEMO: Here, we use the fact that ``the word length of $g_\lambda$
with respect to the relative generating set'' is one, and that is all
what we need. So we may allow that $g_\lambda$ is an element of 
$\bigcup\mathcal{H}$, a part of the relative generating set.}

Therefore,
\[ \dist_{\hat\Gamma}(1, g) \leq \frac{10}{r} \dist_X(x, g.x),\]
if $x\neq g.x$. In general, 
\[ \dist_{\hat\Gamma}(1, g) \leq \frac{10}{r} \dist_X(x, g.x)+5,\]
for any $g\in G$.


For each $H\in \mathcal{H}$, let $x_H\in X$ be a point with $G$-stabilizer equal to $H$. Let $\Phi\colon \hat\Gamma(G,\mathcal{H},S) \to X$ be given by $g\mapsto g.x$ and $gH\mapsto g.x_H$. Let $\lambda=\max\{\dist_X(x,s.x) \colon s\in S\}\cup \{\dist_X(x,x_H)\colon H\in \mathcal{H}\}.$ Then it is an observation that 
\[ \dist_X (x,g.x) \leq \lambda \dist_{\hat\Gamma}(1,g). \]

Since $U_r$ is a ball of radius $r$, $\bigcup_{g\in G} g.U_R=X$ and $\Phi(1)=x\in U_r$, it follows that $\Phi$ is a quasi-isometry.   
\end{proof}

The proof of the above proposition has the following consequence.  
\begin{corollary}
If $G$ acts geometrically relative to a finite collection of subgroups $\mathcal{H}$ on a geodesic metric space $X$, then $G$-orbits in $X$ are discrete. 
\end{corollary}

% \begin{example}
%  Consider the group  $G=\Z\times\Z$ and the subgroup $H=\Z\times \{0\}$. The action of $G$ on the coned-off Cayley graph $X=\hat\Gamma(G,H)$ is geometric relative to $H$. Observe that the fixed point set $X^H$ is not bounded.   
% \end{example}

The following example is to illustrate that in the definition of geodesic coarsely convex group pair, that a relative geometric action on a geodesic space does not imply the additional conditions in the definition.

\begin{example}
 Consider the group  $G=\Z\times\Z\times \Z$ and the subgroups $H=\Z\times\Z\times \{0\}$ and $K=\Z\times\{0\}\times \{0\}$. The action of $G$ on the coned-off Cayley graph $X=\hat\Gamma(G,\{H,K\})$ is geometric relative to the subgroup $H$. This example illustrates that
 \begin{enumerate}[label=$($\alph*$)$]
 \item the fixed point set $X^H$ is not bounded; and 
\item the $G$-stabilizer of any vertex of $X$ of the form $gK$ is neither finite nor a conjugate of $H$.  
\end{enumerate}
\end{example}



==> 65-ConedOffMetricSpaces.tex <==
\label{sec:bicombing_conedoff}

 Let $(X,d_X)$ be a geodesic  metric space, 
let $E$ and $L$ be discrete sets,
$\phi \colon E \to L$ a surjective function and $\psi \colon E \to X$ an injective function with discrete image. 
%or finite image
%isom emb of X 
\[
  \begin{CD}
     E @>{\psi}>> X \\
  @V{\phi}VV     \\
     L.
  \end{CD}
\]
  


%For $\ell>0$, 
The \emph{coned-off space}  $\mathsf{Coned}(X, \psi, \phi)$ is a topological space constructed as follows. 
The underlying space of $\mathsf{Coned}(X, \psi, \phi)$ is the double mapping cylinder of $\phi$ and $\psi$, 
that is, the quotient of $(E\times [0,1]) \sqcup X \sqcup L$ module the relations $(e,0)\sim \psi(e)$ and $(e,\ell)\sim \phi(e)$ for $e\in E$. For $l \in L$, a \emph{cone} $C(l)$ is the image of $\phi^{-1}(l) \times [0,l]$ in the space $\mathsf{Coned}(X,\psi,\phi)$
and a \emph{cone point} is the image of $(\phi^{-1}(l),l)$ in the space $\mathsf{Coned}(X,\psi,\phi,D)$. Regard $\{e\}\times [0,\ell]$ as a segment of length $\ell$ and endow $\mathsf{Coned}(X, \psi, \phi)$ with the induced length metric. 
For $l \in L$, a \emph{cone} $C(l)$ is the image of $\phi^{-1}(l) \times [0,l]$ in the space $\mathsf{Coned}(X,\psi,\phi,D)$
and a \emph{cone point} is the image of $(\phi^{-1}(l),l)$ in the space $\mathsf{Coned}(X,\psi,\phi,D)$. 
%We consider a graph $C(l)$ as the metric space. 
%Each cone $C(l)$ is a uniquely geodesic space with respect to 
We also use the construction in the case that $X$ is a $G$-space ($X$ does not carry a metric, only a topology). 
%In this case, $\ell$ is irrelevant, and the space constructed is denoted as $\mathsf{Coned}(X, \psi, \phi)$.

Observe that the space $\mathsf{Coned}(X,C,x)$ introduced in Section~\ref{sec:const-eqiv-tree} for an $A$-space $X$, a subgroup $C\leq A$ and $x\in X^C$ coincides with $\mathsf{Coned}(X,\psi,\phi)$ where $\phi$ is the identity map on $A/C$, $\psi\colon A/C \to X$ is the $A$-map induced by $C\mapsto x$. Analogously, the space $\mathsf{Coned}(X,H,K,x,y)$ for subgroups $H,K\leq A$ and $x\in X^H$ and $y\in X^K$ arises as $\mathsf{Coned}(X,\psi,\phi)$ where $\phi$ is the identity map on the disjoint union $A/H\sqcup A/K$, and $\psi\colon A/H\sqcup A/K \to X$ is the $A$-map induced by $H\mapsto x$ and $K\mapsto y$.

%The main result of this section states that the sufficient condition of the previous proposition also implies that bicombings on $X$ can be extended to 
%bicombings of $\mathrm{Coned}(X, \psi, \phi, l)$. 


\begin{definition}
We say that the cones in $\mathsf{Coned}(X, \psi, \phi)$ 
are \emph{relatively discrete} if the following two conditions 
are satisfied.
  \begin{enumerate}
    \item For $l_1,l_2\in L$, there exists $z_i\in \psi(\phi^{-1}(l_i))$ for $i=1,2$ such that
        \begin{align*}
            d_X(z_1,z_2) = d_X(\psi(\phi^{-1}(l_1)),\psi(\phi^{-1}(l_2)))
        \end{align*}
      \item For $l\in L$, and $x\in X$, there exists $z\in \psi(\phi^{-1}(l))$ such that
        \begin{align*}
            d_X(x,z) = d_X(x,\psi(\phi^{-1}(l_1)))
        \end{align*}        
\end{enumerate}
%Let $x$ be a cone point
%and let $y$ be points in $X$ or cone points. 
%Assume that 
%there exists a geodesic segment connecting them.
%We call this Condition $(\ast)$.   
\end{definition}

\begin{definition}
 We say that the cones in $\mathsf{Coned}(X, \psi, \phi)$ satisfied the \emph{decreasing geodesic distance condition} if
 for each $l\in L$, the cone $C(l)$ is equipped with a metric $d_l$ such that
  $(C(l),d_l)$ is a geodesic space, and for $e,e'\in \phi^{-1}(l)$ we have
   \begin{align}
    d_X(\psi(e),\psi(e')) \leq d_l((e,1),(e',1))
  \end{align}
\end{definition}

\begin{definition}
    Let $d_l$ be a metric on a cone $C(l)$.
    We say that a family $\{C(l),d_l\}_{l\in L}$ of cones
    is \emph{uniformly radial homogeneous}
    if there exists a constant $D>0$ such that
    for all $l\in L$ 
    and $z\in \psi(\phi^{-1}(l))$, the distance between $z$ 
    and the cone point of $C(l)$  measured by $d_l$ is equal to $D$.
\end{definition}

\begin{proposition}\label{Conedoff-gccbicombing}
 Suppose that each cone $C(l)$ has a metric $d_l$ such that
 the family $\{C(l),d_l\}_{l\in L}$ of cones
 is uniformly radial homogeneous.
 We consider the induced length metric on $\mathsf{Coned}(X,\psi,\phi)$.    \begin{enumerate}
        \item The decreasing geodesic distance condition implies that $X\hookrightarrow \mathsf{Coned}(X,\psi,\phi)$ is an isometric embedding.
        \item The decreasing geodesic distance condition together with cones being relatively discrete in $\mathsf{Coned}(X,\psi,\phi)$ implies that any geodesic bicombing on $X$ can be extended to a geodesic bicombing on $\mathsf{Coned}(X,\psi,\phi)$.
    \end{enumerate}
\end{proposition}



\begin{example}
 The following cases, we have a geodesic metric $d_l$ on $C(l)$
 satisfying all conditions in Proposition \ref{Conedoff-gccbicombing}.
% such that the family $\{C(l),d_l\}_{l\in L}$ is uniformly radial homogeneous, and
% the cones in $\mathsf{Coned}(X, \psi, \phi)$ satisfy 
% the relatively discreteness and the decreasing geodesic distance condition:
 \begin{enumerate}[label=(\Roman*)]
    \item\label{ex:graph}
        For each $l\in L$, $C(l)$ is a discrete space. Then
        $C(l)$ is a graph whose set of edges is $\phi^{-1}(l)$. 
        We endow $C(l)$ with a graph metric $d_l$ such that the length of
        each edge $e\in \phi^{-1}$ is $D>0$, 
        where $D$ a uniform constant. 
        Then $(C(l),d_l)$ is a geodesic space.
        If $D$ satisfies
        \begin{align*}
            \sup \{ d_{X}(\psi(e),\psi(e')) \colon e,e' \in \phi^{-1}(l),\ l \in L \} 
            < D,
        \end{align*} 
        then the decreasing geodesic distance condition is satisfied.
        If the cardinality of 
        $C(l)$ is finite for all $l\in C(l)$, then the cones in 
        $\mathsf{Coned}(X, \psi, \phi)$ are relatively discrete. 
    \item\label{ex:kappa-cone}
        For each $l\in L$, we suppose that 
         $(\psi(\phi^{-1}(l)),d_X)$ is a $\pi$-geodesic space, that is,
         for any $x,y\in \psi(\phi^{-1}(l))$ with $d_X(x,y)< \pi$,
         there exists a geodesic joining $x$ to $y$.
         We define a metric $d_l$ on $C(l)$ by the following formula:
        \begin{align*}
            d_l((x,s),(y,t)) &= (D s)^2 + (D t)^2 -2D^2st 
                \cos(\min\{d_X(x,y), \pi\}) \\
                & \text{for } \quad (x,s),(y,t) \in \psi(\phi^{-1}(l))\times [0,1]
        \end{align*}    
        where $D>0$ is a uniform constant.
        Then by \cite[Chapter I 5.11 Corollary]{MR1744486}, $(C(l),d_l)$ is a geodesic space.
        Moreover, if $D$ satisfies
        \begin{align*}
            \sup \{ d_{X}(\psi(e),\psi(e')) \colon e,e' \in \phi^{-1}(l),\ l \in L \} 
            < D.
        \end{align*} 
        Then the decreasing geodesic distance condition is satisfied.
        If $\psi(\phi^{-1}(l))$ is compact for all $l\in L$, then 
        the cones in 
        $\mathsf{Coned}(X, \psi, \phi)$ are relatively discrete.
%
%        We remark that item \ref{ex:graph} is a special case of 
%        item \ref{ex:Hopf-Rinow}.
%    \item\label{ex:infinite-clique}   
%  Let $X$ be a regular Euclidean simplicial complex, that is, each simplex is isometric to an Euclidean simplex where each side has unit length.    
%    . Let $\{S_l\}$ be a collection of pairwise disjoint (closed) simplices. Consider the $ \mathsf{Coned}(X, \psi, \phi) $ where $E=\bigsqcup_\ell S_l$, $\psi$ is the inclusion. In this case, by the previous item, it is an observation that each cone $C(l)$ satisfies the hypothesis of Proposition~\ref{Conedoff-gccbicombing}, even though the complex  $ \mathsf{Coned}(X, \psi, \phi) $ is not a regular simplicial complex (the metric on each cone $C(l)$ is not Euclidean, it is spherical). Observe that the previous statement holds even if the collection $\{S_l\}$  contains infinite dimensional simplicies since they also have diameter one.
    
%Given a simplicial graph $\Gamma$ and a collection of groups $\mathcal{G}=\{G_u\mid u\in V(\Gamma)\}$, the  \emph{graph product} $\Gamma\mathcal{G}$ is the group arising as the quotient of the free product $\ast_{u\in V(\Gamma) G_u}$ by the normal subgroup generated by all  commutators of the form $[g,h]$ where $g\in G_u$, $h\in G_v$ and $\{u,v\}\in E(\Gamma)$. The Cayley graph  $X(\Gamma, \mathcal G)$ of $\Gamma\mathcal G$ with respect to the generating set $\bigsqcup_{u\in V(\Gamma)} G_u$. It turns out that $X(\Gamma, \mathcal{G})$ is the 1-skeleton of a CAT(0)-complex arising by filling every prism~\cite{}. Note that each coset $gG_u$ for $g\in \Gamma\mathcal{G}$ and $u\in V(\Gamma)$ is the set of vertices of a clique in $X(\Gamma, \mathcal{G})$. 
%\textcolor{red}{Infinite Clique}
 \end{enumerate}
\end{example}

%The assumption~\eqref{D} on the constant $D$ implies that 
\begin{proof}[Proof of Proposition \ref{Conedoff-gccbicombing}]
The decreasing geodesic distance condition implies that
if $\gamma$ is path in  $\mathsf{Coned}(X,\psi,\phi)$ with endpoints in $X$ and the image of $\gamma$ is not contained in $X$, 
then either $\gamma$ backtracks by moving off $X$ towards a cone point and then returning (in particular, it is not injective); 
or pass through a cone point 
and therefore there is a shorter path between the endpoints of $\gamma$ in $\mathsf{Coned}(X,\psi,\phi)$.  
This implies that $X$ is a convex subspace of $\mathsf{Coned}(X,\psi,\phi)$.

%Under Condition $(\ast)$, 
Now we suppose that the cones in $\mathsf{Coned}(X, \psi, \phi)$ are
relatively discrete.
We will show that $\mathsf{Coned}(X,\psi,\phi)$ is a geodesic space. 
$\mathrm{Coned}(X,\psi,\phi)$ is a length space. 
Let $x \in C(l_1)$ and $y \in C(l_2)$. 
We denote by $\gamma$, an path connecting then. 
After $\gamma$ starts from $x$, it either goes up and intersects $X$ via a cone point, or goes down and intersects $X$.
Then $\gamma$ either goes up from $X$, passes through a cone point, goes down, and arrives at $y$, or it goes up from $X$ and arrives at $y$ directly.
Therefore, by assumption, there exists four paths with concatenations of local geodesic segments. 
The shortest path is a geodesic segment connecting $x$ and $y$.  

If $\Gamma$ is a geodesic bicombing on $X$, then $\Gamma$ can be extended to a geodesic bicombing $\hat{\Gamma}$  on $\mathsf{Coned}(X,\psi,\phi)$ defined by~\eqref{eq:def-Gamma-hat-on-Cone}.  

Now let us described the bicombing $\hat \Gamma$. Let $x_1,x_2$ be two distinct points in  $\mathsf{Coned}(X,\psi,\phi)$. If both $x_1,x_2\in X$, we let $\hat\Gamma(x_1,x_2) = \Gamma(x_1,x_2)$.  
 
%The proof of the first part of  Proposition~\ref{Conedoff-gccbicombing} is left to the reader. 
%In the rest of the section, we prove the second statement.

%Under the assumptions of Proposition~\ref{Conedoff-gccbicombing}, we consider $\mathrm{Coned}(X,\psi,\phi,D)$.
%For $l \in L$, a \emph{cone} $C(l)$ is the image of $\phi^{-1}(l) \times [0,D]$ 
%in the space $\mathrm{Coned}(X,\psi,\phi,D)$.
%We consider a graph $C(l)$ as the metric space. 
\begin{comment}
Let $d_l$ be the natural graph metric on $C(l)$. 
A length metric $d$ on $\mathrm{Coned}(X,\psi,\phi,D)$ is as follows:
Let $l_1,l_2 \in L$ such that $l_1 \neq l_2$. 
\begin{itemize}
\item 
If $x \in C(l_1)$ and $y \in C(l_2)$, 
we define
\begin{equation}
\label{inf1}
d(x,y)
= 
\min_{e_1 \in \phi^{-1}(l_1), e_2 \in \phi^{-1}(l_2)} \{
d_{l_1}(x, \psi(e_1)) +
d_{X}(\psi(e_1),\psi(e_2)) +
d_{l_2}(\psi(e_2), y)
\}
\end{equation}

\item 
If $x \in C(l_1)$ and $y \in X$, 
we define
\begin{equation}
\label{inf2}
d(x,y)
= 
\min_{e \in \phi^{-1}(l_1)} \{
d_{l_1}(x, \psi(e)) +
d_{X}(\psi(e),y)
\}
\end{equation}

\item 
If $x, y \in X$, 
we define
\begin{align*}
d(x,y)
= 
d_{X}(x,y) 
\end{align*}
\end{itemize} 
\end{comment}
%Suppose $X$ admits a geodesic bicombing $\Gamma: X \times X \times [0,1] \to X$. 
For each $l \in L$, the cone $C(l)$ is a uniquely geodesic space, so $C(l)$ admits 
the geodesic bicombing
$\Gamma_l \colon C(l) \times C(l) \times [0,1] \to C(l)$.
We define a geodesic bicombing on $\mathsf{Coned}(X,\psi,\phi)$ as follows:
Let $l_1,l_2 \in L$ such that $l_1 \neq l_2$. 
We suppose that $x_1 \in C(l_1)$ and $x_2 \in C(l_2)$.
%Let $x_i=(e_i, t_i)$ for some $e_i \in E_k(l_i)$ and $t_i \in [0,D]$. 
We denote by $\gamma$, a geodesic segment connecting $x_1$ and $x_2$.
Let $e_1 \in \phi^{-1}(l_1)$ and $e_2 \in \phi^{-1}(l_2)$
such that 
$\psi(e_1)$ is the initial point of $\gamma$ in $X$ and
$\psi(e_2)$ is the terminal point of $\gamma$ in $X$.
%which is a geodesic segment connecting $x_1$ and $x_2$
%give 
%the minimum value of the right hand side of \eqref{inf1} for $d(x_1,x_2)$.  
We define
\begin{align}
\label{eq:def-Gamma-hat-on-Cone}
\hat{\Gamma}(x_1,x_2)(t)
 = \left\{
\begin{array}{ll}
\Gamma_{l_1}(x_1, \psi(e_1))\left(t \cdot \dfrac{t_3}{t_1} \right) 
& \left(0 \leq t \leq \dfrac{t_1}{t_3} \right).\\
\Gamma(\psi(e_1), \psi(e_2)) \left( \left( t-\dfrac{t_1}{t_3}\right ) \cdot \dfrac{t_3}{t_2-t_1} \right) 
& \left(\dfrac{t_1}{t_3} \leq t \leq \dfrac{t_2}{t_3} \right). \\
\Gamma_{l_2}(\psi(e_2), x_2) \left( \left( t-\dfrac{t_2}{t_3}\right ) \cdot \dfrac{t_3}{t_3-t_2} \right) 
& \left(\dfrac{t_2}{t_3} \leq t \leq 1 \right). 
\end{array}
\right.
\end{align}
Here $t_1=d_{l_1}(x_1,\psi(e_1))$, 
$t_2=d_{l_1}(x_1,\psi(e_1))+d_X(\psi(e_1),\psi(e_2))$, and 
$t_3=d_{l_1}(x_1,\psi(e_1))+d_X(\psi(e_1),\psi(e_2))+d_{l_2}(\psi(e_2),x_2)$ (see Figure \ref{conesp}).

\end{proof}

%\begin{remark}
%If $\phi^{-1}(\ell)$ is finite for every $\ell\in L$, Condition $(\ast)$ holds.
%\end{remark}

\begin{remark}
For $v,w \in \mathsf{Coned}(X,\psi,\phi)$, the geodesic $\hat{\Gamma}(v,w)$ pass through cones at most twice. 
\end{remark}
%By gluing lemma, $CX$ is a geodesic space. 
\begin{figure}[h]
\begin{tikzpicture}
\draw(0,0)--++(12,0)--++(-1,-1.5)--++(-12,0)--cycle; 
\draw(2,2)node[above]{$l_1$};
\draw(2,2)--++(-1,-2.5);
\draw(1.5,0.75)node[left]{$x_1$};
\fill(1.5,0.75)circle(0.06);
\draw(3,-0.5)node[below]{$\psi(e_1)$};
\draw[very thick](2,2)--++(1,-2.5);
\draw[very thick](3,-0.5)--++(4,0);
\draw[very thick](2,2)--++(-0.5,-1.25);
\fill(3,-0.5)circle(0.06);
\draw(2,2)--++(0,-3);
\draw(2,2)--++(1,-2.5);
%\draw(5,2)node[above]{$\xi^{-1}(l)$};
%\draw(5,2)--++(-1,-2.5);
%\draw(5,2)--++(0,-3);
%\draw(5,2)--++(1,-2.5);
\draw(8,2)node[above]{$l_2$};
\draw(8,2)--++(-1,-2.5);
\draw(7.5,0.75)node[left]{$x_2$};
\fill(7.5,0.75)circle(0.06);
\draw(7,-0.5)node[below]{$\psi(e_2)$};
\draw[very thick](7.5,0.75)--++(-0.5,-1.25);
\fill(7,-0.5)circle(0.06);
\draw(8,2)--++(0,-3);
\draw(8,2)--++(1,-2.5);
\end{tikzpicture}
\caption{The bold line is an schematic of a geodesic $\hat{\Gamma}(x_1,x_2)$ provided by the bicombing $\hat\Gamma$.}
\label{conesp}
\end{figure}
%%%
\begin{comment}
\begin{proposition}
%Let $\hat{\Gamma}$ be a geodesic bicombing on $\mathrm{Coned}(X,\psi,\phi,D)$ constructed in the above. 
If $\Gamma$ is a geodesic coarsely convex bicombing on $X$, 
then $\hat{\Gamma}$ is a geodesic coarsely convex bicombing on $\mathrm{Coned}(X,\psi,\phi,D)$.
\end{proposition}
\end{comment}

\begin{theorem}
\label{conedOff-bicombing-convex}
    %Suppose that Condition $(\ast)$ holds.
    %Suppose that a family of metrics $d_l$ on the cones $C(l)$ $(l\in L)$ is uniformly radial homogeneous.
    Suppose that each cone $C(l)$ has a metric $d_l$ such that the family $\{C(l),d_l\}_{l\in L}$ of cones is uniformly radial homogeneous.
    The decreasing geodesic distance condition together with cones being relatively discrete in $\mathsf{Coned}(X,\psi,\phi)$ implies that
    if $\Gamma$ is geodesic coarsely convex,
    then $\hat{\Gamma}$ is geodesic coarsely convex
\end{theorem}

We prove Theorem~\ref{conedOff-bicombing-convex} 
by invoking Theorem~\ref{consistent-and-thin-cconvex} which has three assumptions that are verified in the following three lemmas.
In these three lemmas, 
we assume that $\Gamma$ satisfies the hypotheses of Theorem~\ref{conedOff-bicombing-convex}.
%$\Gamma$ satisfies Condition $(\ast)$ is assumed

\begin{lemma}
If $\Gamma$ is coarsely consistent, 
then $\hat{\Gamma}$ is coarsely consistent.
\end{lemma}

\begin{lemma}
\label{cocft}
%If $\Gamma$ is a geodesic coarsely convex bicombing on $X$, 
If $\Gamma$ is geodesic coarsely convex,
then $\hat{\Gamma}$ is coarsely forward thin.
\end{lemma}

\begin{lemma}
\label{cocbt}
If $\Gamma$ is geodesic coarsely convex,
then $\hat{\Gamma}$ is coarsely backward thin.
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{cocft}]
$\Gamma$ is uniformly radial homogeneous with a constant $D$. 
The decreasing geodesic distance condition implies that for each $l \in L$,
\begin{align*}
    \mathrm{diam}(\psi(\phi^{-1}(l))) \leq 2D
\end{align*}
holds.
Suppose $\Gamma$ is a geodesic $(E,C)$-coarsely convex bicombing. 
The conclusion of the lemma follows by verifying the hypotheses of Definition~\ref{cftd}.
%Suppose 
%\begin{align*}
%    \min\{d(v,w_1), d(v,w_2)\}\geq 2D. 
%\end{align*}
Proposition~\ref{Conedoff-gccbicombing} implies that $X$ is a convex space of $\mathsf{Coned}(X,\psi,\phi)$.
%%%%
$\hat{\Gamma}$ restricted to $X \times X$ is a geodesic $(E,C)$-coarsely convex bicombing. 
%%%%
To simplify notation, let $CX$ denote $\mathrm{Coned}(X,\psi,\phi)$. 
Let $v,w_1,w_2 \in CX$. We suppose that one of $v,w_1,w_2$ is contained in
a cone $C(l)$ and the set $\{v,w_1,w_2\}$ is not contained in $C(l)$.
Let $\gamma_1=\hat{\Gamma}(v,w_1)$ and $\gamma_2=\hat{\Gamma}(v,w_2)$. 
\par
First, we will show that $\hat{\Gamma}$ satisfies 
%the assumption (\ref{ccgccc1}) of Lemma \ref{ccgccc}.
Item (\ref{Ex-3-2}) of Definition~\ref{cftd}.
%We consider the following three cases:
%The intersection of the $\gamma_1$ and $\gamma_2$ with the convex subspace $X$ yields two geodesics given by the combing $\Gamma$ whose initial points are at distance at most $2D$ in $X$, 
%and terminal points are also at distance at most $2D$ in $X$
%For $x,y \in CX$, let $[x,y]$ be the image of $\hat{\Gamma}(x,y)$.
%The geodesic triangle $[\gamma_1(0),\gamma_1(1)] \cup [\gamma_1(1),\gamma_2(1)] \cup [\gamma_2(1),\gamma_1(0)]$ has the following form (see Figure \ref{geodtri}).
Suppose $v$ belongs to the cone $C(l)$. 
Since $w_1$ and $w_2$ are not in $C(l)$, the geodesic $\gamma_1$ intersects the convex subspace $X$ in a geodesic that we denote by $\gamma_1\cap X$. 
Let $p_1$ the initial point of $\gamma_1\cap X$ on $X$; analogously, let $p_2$ the initial point of $\gamma_2$ on $X$. 
Let $a$ be the terminal point of the geodesic $\gamma_1\cap X$  
and let $b$ be the terminal point of the geodesic $\gamma_2\cap X$.  
Define the parameters $c_0,c_1,c_0'$ and $c_1'$ in $[0,1]$  by
\[ p_1=\gamma_1(c_0),\quad a=\gamma_1(c_1),\quad p_2=\gamma_2(c_0^{\prime}),\quad b=\gamma_2(c_1^{\prime}) ,\]
%In the case that $v$ does not belong to a cone, we let $p_1=v$ and $p_2=v$. 
%In any case, 
%$d(p_1,p_2)\leq 2D$ since the cones have diameter $2D$.  
The reparametrization of $\gamma_1|_{[0,c_0]}$ and $\gamma_2|_{[0,c_0']}$ coarsely $2D$-fellow travel since the cones have diameter $2D$. 
%$\gamma_1\cap X$ and $\gamma_2\cap X$ coarsely $2D$-fellow travel since the cones have diameter $2D$. 
%Let $a$ be the terminal point of the geodesic $\gamma_1\cap X$  
%and let $b$ be the terminal point of the geodesic $\gamma_2\cap X$.  
\par
The geodesics $\gamma_1$ and $\gamma_2$ can be expressed as concatenations of $\Gamma$ on $X$ and the geodesic bicombings on cones.
%\begin{gather*}
%[\gamma_1(0), \gamma_1(1)]= [\gamma_1(0), p_1] \cup [p_1,a] \cup [a, \gamma_1(1)], \\ 
%[\gamma_1(0), \gamma_2(1)]= [\gamma_1(0), p_2] \cup [p_2,b] \cup [b, \gamma_2(1)], \mathrm{and}, \\
%d(\gamma_1(1), \gamma_2(1))= d(\gamma_1(1), a) + d(a,b) + d(b, \gamma_2(1)).  
%\end{gather*}
Thus, the image of $\gamma_1 \cap X$ coincides with that of $\Gamma(p_1,a)$
and the image of $\gamma_2 \cap X$ coincides with that of $\Gamma(p_2,b)$.
%Define the parameters $c_0,c_1,c_0'$ and $c_1'$ in $[0,1]$  by
%\[ p_1=\gamma_1(c_0),\quad a=\gamma_1(c_1),\quad p_2=\gamma_2(c_0^{\prime}),\quad b=\gamma_2(c_1^{\prime}) ,\]
%and let 
Item (\ref{Ex-3-4}) of Definition~\ref{cftd} holds.
\par
Next, we will show that Item (\ref{Ex-3-5}) of Definition~\ref{cftd} holds.
%In the case that $w_1 \in X$ and $w_2$ belongs to the cone, we let $a=w_1$.
%Since $X$ is a convex subspace of $CX$, we have
%\begin{align*}
%    d_{CX}(w_1,w_2)&=d_{CX}(a,w_2) \\
%                   &=d_{CX}(a,b)+d_{CX}(b,w_2).                
%\end{align*}
%%%
%Suppose that both $w_1$ and $w_2$ belong to cones. 
In the case that $w_1$ and $w_2$ belong to the same cone, It is clear that Item (\ref{Ex-3-4}) of Definition~\ref{cftd} holds.
%Let $\eta=\hat{\Gamma}(\gamma_1(1),\gamma_2(1))$. 
Suppose that $w_1$ and $w_2$ belong to distinct cones,
the geodesic $\eta=\hat{\Gamma}(w_1,w_2)$ intersects the convex subspace $X$ in a geodesic that we denote by $\eta\cap X$. 
Let $q_1$ the initial point of $\eta \cap X$ on $X$
and let $q_2$ be the terminal point of $\gamma_1\cap X$.
Since the cones have diameter $2D$, we have
\begin{align*}
 d_{CX}(q_1,a) < 2D\quad \text{and} \quad d_{CX}(q_2,b)<2D.
\end{align*}
By the triangle inequality implies that
\begin{align}
    &d_{CX}(w_1,a)+d_{CX}(a,b)+d_{CX}(b,w_2) \notag \\
    &\leq d_{CX}(w_1,q_1)+2D +d_{CX}(q_1,q_2)+4D +d_{CX}(q_2,w_2)+2D \notag \\
    &=d_{CX}(w_1,w_2)+8D. \label{w1w2}
\end{align}
In any case, Item (\ref{Ex-3-5}) of Definition~\ref{cftd} holds.
\par
%Since $d(p_1, p_2)\leq 2D$, we have $|c_0t-c_0^{\prime}s| \leq 2D$. 
%By considering a geodesic between $\gamma_1(1)$ and $\gamma_2(1)$, and taking into account that cones have diameter $2D$, 
Inequality \eqref{w1w2} implies
\begin{align*}
&c_1^{\prime} \cdot d(\gamma_1(1), \gamma_2(1)) - d(a,b) \\
%&=c_1^{\prime}\{ d(\gamma_1(1), a) + d(a,b) + d(b, \gamma_2(1))\} - d(a,b)\\
%&=c_1^{\prime}d(\gamma_1(1), a) + c_1^{\prime}d(b, \gamma_2(1)) - (1-c_1^{\prime})d(a,b) \\
&\geq c_1^{\prime}d(\gamma_1(1), \gamma_1(c_1)) + c_1^{\prime}d(\gamma_2(c_1^{\prime}), \gamma_2(1)) - (1-c_1^{\prime})d(a,b) 
-8D\\
&=c_1^{\prime}(1-c_1)d(\gamma_1(1), \gamma_1(0)) + c_1^{\prime}(1-c_1^{\prime})d(\gamma_2(0), \gamma_2(1)) - (1-c_1^{\prime})d(a,b) -4D. 
\end{align*}
Without loss of generality, assume that $c_1 \leq c_1^{\prime}$.
Then the right-hand side of this inequality can be estimated as follows:
\begin{align*}
& c_1^{\prime}(1-c_1)d(\gamma_1(1), \gamma_1(0)) + c_1^{\prime}(1-c_1^{\prime})d(\gamma_2(0), \gamma_2(1)) - (1-c_1^{\prime})d(a,b) -8D\\
&\geq c_1^{\prime}(1-c_1^{\prime})d(\gamma_1(1), \gamma_1(0)) + c_1^{\prime}(1-c_1^{\prime})d(\gamma_2(0), \gamma_2(1)) - (1-c_1^{\prime})d(a,b) -8D\\
&= (1-c_1^{\prime})\{ c_1^{\prime}d(\gamma_1(1), \gamma_1(0)) + c_1^{\prime}d(\gamma_2(0), \gamma_2(1)) - d(a,b)\} -8D\\
&\geq (1-c_1^{\prime})\{ c_1d(\gamma_1(1), \gamma_1(0)) + c_1^{\prime}d(\gamma_2(0), \gamma_2(1)) - d(a,b)\} -8D\\
&= (1-c_1^{\prime})\{ d(a, \gamma_1(0)) + d(\gamma_2(0),b) - d(a,b)\} -8D\\
&\geq -8D.
\end{align*}
The last inequality follows from the triangle inequality.
Then, we obtain that Item (\ref{Ex-3-3}) of Definition~\ref{cftd} hplds. 
%\[
% d(a,b) \leq c_1^{\prime} \cdot d(\gamma_1(1), \gamma_2(1)) +4D. \qedhere
%\]
\end{proof}

Lemma~\ref{cocbt} can be proved in the same manner as Lemma~\ref{cocft}. 

\begin{comment}
\begin{enumerate}
\item\label{ecase1}
The distances $d(v,w_1), d(v,w_2), d(w_1,w_2)$ are larger or equal to $2D$.
\item\label{ecase2}
At least one of the distances $d(v,w_1), d(v,w_2)$ is less than $2D$.
\item $\min\{d(v,w_1), d(v,w_2)\}\geq 2D$ and  $d(w_1,w_2)<2D$.
\end{enumerate}
In the second case, one of the geodesics $\gamma_1, \gamma_2$ has length less than $2D$ and it is an exercise to verify that assumption (\ref{ccgccc1}) of Lemma \ref{ccgccc} holds.  In the third case, the intersection of the $\gamma_1$ and $\gamma_2$ with the convex subspace $X$ yields two geodesics given by the combing $\Gamma$ whose initial points are at distance at most $2D$ in $X$, and terminal points are also at distance at most $2D$ in $X$; then the geodesic coarsely convex property of $\Gamma$ implies assumption (\ref{ccgccc1}) of Lemma \ref{ccgccc} for $\gamma_1$ and $\gamma_2$. Below, we discuss in detail the first case. 

 
For $x,y \in CX$, let $[x,y]$ be the image of $\hat{\Gamma}(x,y)$.
The geodesic triangle $[\gamma_1(0),\gamma_1(1)] \cup [\gamma_1(1),\gamma_2(1)] \cup [\gamma_2(1),\gamma_1(0)]$ has the following form (see Figure \ref{geodtri}).
Suppose $v$ belongs to a cone $C(l)$. Since $d(v,w_1)\geq 2D$, the geodesic $\gamma_1$ intersects the convex subspace $X$ in a geodesice that we denote by $\gamma_1\cap X$. Let $p_1$ the initial point of $\gamma_1\cap X$ on $X$; analogously, let $p_2$ the initial point of $\gamma_2$ on $X$. In the case that $v$ does not belong to a cone, we let $p_1=v$ and $p_2=v$. In any case, $d(p_1,p_2)\leq 2D$ since the cones have diameter $2D$.  Let $a$ be the terminal point of the geodesic $\gamma_1\cap X$  and let $b$ be the terminal point of the geodesic $\gamma_2\cap X$.  The geodesics $\gamma_1$ and $\gamma_2$ can be expressed as concatenations 
\begin{gather*}
[\gamma_1(0), \gamma_1(1)]= [\gamma_1(0), p_1] \cup [p_1,a] \cup [a, \gamma_1(1)], \\ 
[\gamma_1(0), \gamma_2(1)]= [\gamma_1(0), p_2] \cup [p_2,b] \cup [b, \gamma_2(1)], \mathrm{and}, \\
d(\gamma_1(1), \gamma_2(1))= d(\gamma_1(1), a) + d(a,b) + d(b, \gamma_2(1)).  
\end{gather*}
Define the parameters $c_0,c_1,c_0'$ and $c_1'$ in $[0,1]$  by
\[ p_1=\gamma_1(c_0),\quad a=\gamma_1(c_1),\quad p_2=\gamma_2(c_0^{\prime}),\quad b=\gamma_2(c_1^{\prime}) ,\]
and let 
%%%
%\begin{figure}[h]
%\begin{tikzpicture}
%\draw(0,0)--++(6,0)--++(-1,-1.5)--++(-6,0)--cycle; 
%\draw(5,-1.5)node[below]{$CX_k$};
%\draw[dashed](1,-1)--++(-0.5,-0.5);
%\draw(0.5,-1.5)--++(-1.5,-1.5);
%\draw(-1,-3)node[below]{$\gamma_1(0)$};
%\fill(-1,-3)circle(0.06);
%\draw(1,-1)--++(2,0.75)--++(0.75,-0.75)--cycle;
%\draw(1,-1)node[below]{$p$};
%\draw(3.5,-0.25)node[left]{$a$};
%\draw(3.75,-1)node[below]{$b$};
%\draw(3,-0.25)--++(1,2);
%\draw(4,1.75)node[above]{$\gamma_1(1)$};
%\fill(4,1.75)circle(0.06);
%\draw(3.75,-1)--++(3,1);
%\draw(6.75,0)node[above]{$\gamma_2(1)$};
%\fill(6.75,0)circle(0.06);
%\end{tikzpicture}
%\caption{In case ii), an example of geodesic triangles of $\mathsf{Z}$.}
%\label{gt}
%\end{figure}
%%%%
%%%%
\begin{figure}[t]
\begin{tikzpicture}
\draw(0,0.5)--++(2,0.5)--++(0,-2)--++(-2,0.5)--cycle;
\draw(-3,0)--++(3,0.5);
\draw(-3,0)--++(3,-0.5);
\draw(-3,0)node[left]{$\gamma_1(0)$};
\draw(0,0.5)node[above]{$p_1$};
\draw(0,-0.5)node[below]{$p_2$};
\fill(-3,0)circle(0.06);
\draw(2,1)--++(1,1.5);
\draw(2,1)node[above]{$a$};
\draw(3,2.5)node[above]{$\gamma_1(1)$};
\fill(3,2.5)circle(0.06);
\draw(2,-1)--++(1,-1.5);
\draw(2,-1)node[right]{$b$};
\draw(3,-2.5)node[below]{$\gamma_2(1)$};
\fill(3,-2.5)circle(0.06);
%%%
%\draw(1,0.75)node[above]{$\gamma_1(c)$};
%\fill(1,0.75)circle(0.06);
%\draw(1,-0.75)node[below]{$\gamma_2(c)$};
%\fill(1,-0.75)circle(0.06);
\end{tikzpicture}
\caption{Case (\ref{ecase1})}
\label{geodtri}
\end{figure}
%%%%
\[ t=d(\gamma_1(0),\gamma_1(1)), \qquad s=d(\gamma_2(0),\gamma_2(1)).\]
\end{comment}

\begin{comment}
\begin{lemma}\label{key3}
% We have the following inequality.
 $d(a,b) \leq \max\{c_1,c_1^{\prime}\} d(\gamma_1(1), \gamma_2(1)) +4D.$
\end{lemma}
\begin{proof}
%Since $d(p_1, p_2)\leq 2D$, we have $|c_0t-c_0^{\prime}s| \leq 2D$. 
By considering a geodesic between $\gamma_1(1)$ and $\gamma_2(1)$, and taking into account that cones have diameter $2D$, the triangle inequality implies
\begin{align*}
&c_1^{\prime} \cdot d(\gamma_1(1), \gamma_2(1)) - d(a,b) \\
%&=c_1^{\prime}\{ d(\gamma_1(1), a) + d(a,b) + d(b, \gamma_2(1))\} - d(a,b)\\
%&=c_1^{\prime}d(\gamma_1(1), a) + c_1^{\prime}d(b, \gamma_2(1)) - (1-c_1^{\prime})d(a,b) \\
&\geq c_1^{\prime}d(\gamma_1(1), \gamma_1(c_1)) + c_1^{\prime}d(\gamma_2(c_1^{\prime}), \gamma_2(1)) - (1-c_1^{\prime})d(a,b) 
-4D\\
&=c_1^{\prime}(1-c_1)d(\gamma_1(1), \gamma_1(0)) + c_1^{\prime}(1-c_1^{\prime})d(\gamma_2(0), \gamma_2(1)) - (1-c_1^{\prime})d(a,b) -4D. 
\end{align*}
Without loss of generality, assume that $c_1 \leq c_1^{\prime}$.
Then the right-hand side of this inequality can be estimated as follows:
\begin{align*}
& c_1^{\prime}(1-c_1)d(\gamma_1(1), \gamma_1(0)) + c_1^{\prime}(1-c_1^{\prime})d(\gamma_2(0), \gamma_2(1)) - (1-c_1^{\prime})d(a,b) -4D\\
&\geq c_1^{\prime}(1-c_1^{\prime})d(\gamma_1(1), \gamma_1(0)) + c_1^{\prime}(1-c_1^{\prime})d(\gamma_2(0), \gamma_2(1)) - (1-c_1^{\prime})d(a,b) -4D\\
&= (1-c_1^{\prime})\{ c_1^{\prime}d(\gamma_1(1), \gamma_1(0)) + c_1^{\prime}d(\gamma_2(0), \gamma_2(1)) - d(a,b)\} -4D\\
&\geq (1-c_1^{\prime})\{ c_1d(\gamma_1(1), \gamma_1(0)) + c_1^{\prime}d(\gamma_2(0), \gamma_2(1)) - d(a,b)\} -4D\\
&= (1-c_1^{\prime})\{ d(a, \gamma_1(0)) + d(\gamma_2(0),b) - d(a,b)\} -4D\\
&\geq -4D.
\end{align*}
The last inequality follows from the triangle inequality.
Then, we obtain the desired inequality. 
%\[
% d(a,b) \leq c_1^{\prime} \cdot d(\gamma_1(1), \gamma_2(1)) +4D. \qedhere
%\]
\end{proof}
\end{comment}

\begin{comment}
\par 
We will show that 
there exist $E_{*} \geq 1$ and $C_* \geq 0$ depending only on $E$ and $C$ such that
for all $c \in [0,1]$, 
\begin{align*} 
d(\gamma_1(c), \gamma_2(c)) \leq cE_*d(\gamma_1(1), \gamma_2(1))+C_*.
\end{align*}
We divide the proof into the following cases: 
\begin{enumerate}
\renewcommand{\labelenumi}{\roman{enumi}).}
\item \label{eitem0)} 
    $\gamma_1(c) \in [\gamma_1(0),p_1]$ or $\gamma_2(c) \in [\gamma_1(0),p_2]$.
\item \label{eitemI)} 
    $\gamma_1(c) \in [p_1,a]$ and $\gamma_2(c) \in [p_2,b]$ (see Figure \ref{eI)}).
%\item \label{eitemI)} $\gamma_1(c) \in [p_1,a]$ and $\gamma_2(c) \in [p_2,b]$ (see Figure \ref{I)}).
\item \label{eitemII)}
    $\gamma_1(c) \in [p_1,a]$ and $\gamma_2(c) \in [b, \gamma_2(1)]$ %(see Figure \ref{eII)}).
\item \label{eitem-III}
    $\gamma_1(c) \in [a, \gamma_1(1)]$ and $\gamma_2(c) \in [b, \gamma_2(1)]$ %(see Figure \ref{eIII)}).
\end{enumerate}

\par 
In case i), we suppose $\gamma_1(c) \in [\gamma_1(0),p_1]$. 
Since $\gamma_1(c)$ and $p_2$ are in the same cone, we have 
\begin{align*}
d(\gamma_1(c),p_2) \leq 2D. 
\end{align*}
Moreover, Since $\hat{\Gamma}$ is a geodesic bicombing, 
\begin{align*}
|ct-c_0's| \leq 2D
\end{align*}
holds. 
Combing these inequalities and the triangle inequality, we have 
\begin{align*}
d(\gamma_1(c),\gamma_2(c) 
&\leq d(\gamma_1(c),p_2) +d(p_2,\gamma_2(c)) \\
&\leq 2D +d(\gamma_2(c_0'),\gamma_2(c)) \\
&\leq |c_0's-cs| + 2D \\
&\leq |c_0's-ct|+|ct-cs| +2D \\
&\leq c|t-s| +4D \\
&\leq cd(\gamma_1(1),\gamma_2(1)) +4D. 
\end{align*}

\par 
In case ii), we can put
\begin{align*}
\gamma_1(c)&=\Gamma(p_1,a)\left( \dfrac{c-c_0}{c_1-c_0}\right), \\
\gamma_2(c)& =\Gamma(p_2,b)\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}\right).
\end{align*}
%%%
%\begin{figure}[h]
%\begin{tikzpicture}
%\draw(0,0)--++(2,1)--++(0,-2)--cycle;
%\draw(-2,0)--++(2,0);
%\draw(-2,0)node[left]{$\gamma_1(0)$};
%\draw(0,0)node[above]{$p$};
%\fill(-2,0)circle(0.06);
%\draw(2,1)--++(1,1.5);
%\draw(2,1)node[above]{$a$};
%\draw(3,2.5)node[above]{$\gamma_1(1)$};
%\fill(3,2.5)circle(0.06);
%\draw(2,-1)--++(1,-1.5);
%\draw(2,-1)node[right]{$b$};
%\draw(3,-2.5)node[below]{$\gamma_2(1)$};
%\fill(3,-2.5)circle(0.06);
%%%
%\draw(1,0.5)node[above]{$\gamma_1(c)$};
%\fill(1,0.5)circle(0.06);
%\draw(1,-1)node{$\gamma_2(c)$};
%\fill(1,-0.5)circle(0.06);
%\end{tikzpicture}
%\caption{Case I)}
%\label{I)}
%\end{figure}
%%%
%%%
\begin{figure}[h]
\begin{tikzpicture}
\draw(0,0.5)--++(2,0.5)--++(0,-2)--++(-2,0.5)--cycle;
\draw(-3,0)--++(3,0.5);
\draw(-3,0)--++(3,-0.5);
\draw(-3,0)node[left]{$\gamma_1(0)$};
\draw(0,0.5)node[above]{$p_1$};
\draw(0,-0.5)node[below]{$p_2$};
\fill(-3,0)circle(0.06);
\draw(2,1)--++(1,1.5);
\draw(2,1)node[above]{$a$};
\draw(3,2.5)node[above]{$\gamma_1(1)$};
\fill(3,2.5)circle(0.06);
\draw(2,-1)--++(1,-1.5);
\draw(2,-1)node[right]{$b$};
\draw(3,-2.5)node[below]{$\gamma_2(1)$};
\fill(3,-2.5)circle(0.06);
%%%
\draw(1,0.75)node[above]{$\gamma_1(c)$};
\fill(1,0.75)circle(0.06);
\draw(1,-0.75)node[below]{$\gamma_2(c)$};
\fill(1,-0.75)circle(0.06);
\end{tikzpicture}
\caption{Case II)}
\label{eI)}
\end{figure}
%%%
%Set $T\coloneqq(c_1-c_0)t$ and $S\coloneqq(c_1^{\prime}-c_0^{\prime})s$.
%Then we have
Note that
\begin{align*}
p_1&=\Gamma(p_1,a)(0), & p_2 &=\Gamma(p_2,b)\left( 0 \right), \\
\gamma_1(c)&=\Gamma(p_1,a)\left( \dfrac{c-c_0}{c_1-c_0}\right),                                     & a &=\Gamma(p_1,a)\left(1\right), \\ 
\gamma_2(c)&=\Gamma(p_2,b)\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}\right), & b &=\Gamma(p_2,b)\left(1\right).
\end{align*}
We define $a^{\prime} \in [p_1,a]$ to be
\begin{align*}
a^{\prime}\coloneqq \Gamma(p_1,a)\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}\right).
\end{align*}
First, since $\Gamma$ is a geodesic $(E,C)$-coarsely convex bicombing, by Inequality \eqref{key3}, we have
\begin{align}
d(a^{\prime}, \gamma_2(c)) 
&=d \left( \Gamma(p_1,a)\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}\right) , \Gamma(p_2,b)\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}\right) \right)  \notag \\
&\leq \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} \cdot Ed(\Gamma(p_1,a)(1), \Gamma(p_2,b)(1))  \notag \\
&\ + \left( 1- \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} \right) \cdot Ed(\Gamma(p_1,a)(0), \Gamma(p_2,b)(0)) +C\notag \\
&= \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} \cdot Ed(a, b) +\left( 1- \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} \right)Ed(p_1,p_2) +C\notag \\
&\leq \dfrac{cc_1^{\prime}-c_0^{\prime}c_1^{\prime}}{c_1^{\prime}-c_0^{\prime}} \cdot Ed(\gamma_1(1), \gamma_2(1)) +4D +2ED +C\label{c2-0} \\
&\leq c \cdot Ed(\gamma_1(1), \gamma_2(1)) +4D+ 2ED +C. \label{c2-1}
\end{align}
Inequality \eqref{c2-0} follows from Lemma \ref{key3} and
Inequality \eqref{c2-1} follows from $c_0^{\prime} \leq c \leq c_1^{\prime}$.

\par 
Next, we consider the distance between $a^{\prime}$ and $\gamma_1(c)$.
Then
\begin{align*}
d(a^{\prime}, \gamma_1(c)) 
&=d \left( \Gamma(p_1,a)\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}\right) , \Gamma(p_1,a)\left( \dfrac{c-c_0}{c_1-c_0}\right) \right)  \notag \\
&=\left| \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} -\dfrac{c-c_0}{c_1-c_0}\right| \cdot d(p_1,a) \notag \\
&=\left| \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} -\dfrac{c-c_0}{c_1-c_0}\right| \cdot (c_1-c_0)t. \notag 
\end{align*}
By the triangle inequality $ (c_1-c_0)t  \leq (c_1^{\prime}-c_0^{\prime})s+ d(a,b)+ d(p_1,p_2)$, and $|c_0t-c_0's| \leq 2D$, and Lemma \ref{key3}, we have
\begin{align*}
\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} -\dfrac{c-c_0}{c_1-c_0} \right)(c_1-c_0)t 
&=\dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} (c_1-c_0)t  -\dfrac{c-c_0}{c_1-c_0}(c_1-c_0)t   \\
&\leq \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}  \{ (c_1^{\prime}-c_0^{\prime})s+ d(a,b) +d(p_1,p_2)\} -(c-c_0)t   \\
&\leq (c-c_0^{\prime})s -(c-c_0)t +\dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} d(a,b) +\dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} d(p_1,p_2)\\
&\leq c(s-t) + (c_0t-c_0^{\prime}s) +cd(\gamma_1(1),\gamma_2(1)) +D \\
&\leq c \cdot \{2d(\gamma_1(1), \gamma_2(1))\} +3D.
\end{align*}
Similarly, by the triangle inequality $ (c_1^{\prime}-c_0^{\prime})s - d(a,b)-d(p_1,p_2)  \leq  (c_1-c_0)t$, and $|c_0t-c_0's| \leq 2D$, and Inequality \eqref{key3}, we have
\begin{align*}
\left( \dfrac{c-c_0}{c_1-c_0} - \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} \right) (c_1-c_0)t 
&=\dfrac{c-c_0}{c_1-c_0}(c_1-c_0)t  - \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} (c_1-c_0)t  \\
&\leq (c-c_0)t -\dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}  \{ (c_1^{\prime}-c_0^{\prime})s - d(a,b)-d(p_1,p_2)\} \\
&= (c-c_0)t - (c-c_0^{\prime})s +\dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} d(a,b) +\dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}d(p_1,p_2) \\
&\leq c(t-s) + (c_0's-c_0t) +cd(\gamma_1(1),\gamma_2(1)) +D\\
&\leq c \cdot \{2d(\gamma_1(1), \gamma_2(1))\} +3D.
\end{align*}
Then we have
\begin{align}
d(a^{\prime}, \gamma_1(c))
&=\left| \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} -\dfrac{c-c_0}{c_1-c_0}\right| \cdot (c_1-c_0)t \notag \\
&\leq c \cdot \{2d(\gamma_1(1), \gamma_2(1))\} +3D. \label{2-2}
\end{align}
Combining \eqref{c2-1} and \eqref{2-2} yields
\begin{align*}
d(\gamma_1(c),\gamma_2(c)) 
&\leq d(\gamma_1(c),a^{\prime}) + d(a^{\prime}, \gamma_2(c)) \\ 
& \leq c \cdot \{2d(\gamma_1(1), \gamma_2(1))\} + c \cdot Ed(\gamma_1(1), \gamma_2(1)) +ED +3D +C \\
& = c(2+E) d(\gamma_1(1), \gamma_2(1)) +ED +3D +C.
\end{align*}
\end{comment}

\begin{comment}
In case III), we supposed that $\gamma_1(c) \in [p_1,a]$ and $\gamma_2(c) \in [b, \gamma_2(1)]$,
where $a=\gamma_1(c_1)$ and $b=\gamma_2(c^{\prime}_1)$.
Let  $t^{\prime} \coloneqq c_1$ and $s^{\prime} \coloneqq c^{\prime}_1$.
We define
\begin{gather*}
a^{\prime} \coloneqq \gamma_1(ct^{\prime}), \\ 
b^{\prime} \coloneqq \gamma_2(cs^{\prime}).
\end{gather*}
\begin{figure}[h]
\begin{tikzpicture}
\draw(0,0.5)--++(2,0.5)--++(0,-2)--++(-2,0.5)--cycle;
\draw(-3,0)--++(3,0.5);
\draw(-3,0)--++(3,-0.5);
\draw(-3,0)node[left]{$\gamma_1(0)$};
\draw(0,0.5)node[above]{$p_1$};
\draw(0,-0.5)node[below]{$p_2$};
\fill(-3,0)circle(0.06);
\draw(2,1)--++(1,1.5);
\draw(2,1)node[above]{$a$};
\draw(3,2.5)node[above]{$\gamma_1(1)$};
\fill(3,2.5)circle(0.06);
\draw(2,-1)--++(1,-1.5);
\draw(2,-1)node[right]{$b$};
\draw(2.5,-1.75)node[right]{$\gamma_2(c)$};
\fill(2.5,-1.75)circle(0.06);;
\draw(3,-2.5)node[below]{$\gamma_2(1)$};
\fill(3,-2.5)circle(0.06);
%%
\draw(0.5,0.625)node[below]{$a'$};
\fill(0.5,0.625)circle(0.06);
\draw(1,0.75)node[above]{$\gamma_1(c)$};
\fill(1,0.75)circle(0.06);
\draw(1,-0.75)node[below]{$b'$};
\fill(1,-0.75)circle(0.06);
\end{tikzpicture}
\caption{Case III)}
\label{eII)}
\end{figure}
Since $a=\gamma_1(t^{\prime})$ and $b=\gamma_2(s^{\prime})$, we have $a^{\prime} \in [\gamma_1(0), p_1] \cup [p_1,a]$ and $b^{\prime} \in [\gamma_1(0), p_2] \cup [p_2,b]$.
By the same argument as in case II), we have
\begin{align*}
d(a^{\prime}, b^{\prime})
&=d(\gamma_1(ct^{\prime}), \gamma_2(cs^{\prime}) ) \\
&\leq  c(2+E) d(\gamma_1(t^{\prime}), \gamma_2(s^{\prime})) +ED +4D +C \\
&=c(2+E) d(a,b) +ED +4D +C.
\end{align*}
We remark that $d(\gamma_1(1),\gamma_2(1)) = d(\gamma_1(1),a)+d(a,b)+d(b,\gamma_2(1))$.
Then we have
\begin{align*}
&d(\gamma_1(c), \gamma_2(c)) \\
& \leq d(\gamma_1(c), a^{\prime}) + d(a^{\prime},b^{\prime}) +d(b^{\prime}, \gamma_2(c)) \\
& = d(\gamma_1(c), \gamma_1(ct^{\prime}) )+ d(\gamma_1(ct^{\prime}),\gamma_2(cs^{\prime}))+d(\gamma_2(cs^{\prime} ), \gamma_2(c)) \\
&\leq c(1-t^{\prime})t + c(2+E) d(\gamma_1(t^{\prime}), \gamma_2(s^{\prime})) +ED +4D +C + c(1-s^{\prime})s \\
&= cd(\gamma_1(1),\gamma_1(t^{\prime})) +c(2+E) d(\gamma_1(t^{\prime}), \gamma_2(s^{\prime})) + ED + 4D +C + cd(\gamma_2(s^{\prime}), \gamma_2(1)) \\
&\leq c(2+E) \{ d(\gamma_1(1), a) + d(a,b) + d(b, \gamma_2(1)) \} +ED +4D +C \\
&= c(2+E) d(\gamma_1(1),\gamma_2(1)) +ED +4D  +C. 
\end{align*}
\par 
We consider case IV).
In case IV), we supposed that $\gamma_1(c) \in [a, \gamma_1(1)]$ and $\gamma_2(c) \in [b, \gamma_2(1)]$,
where $a=\gamma_1(c_1)$, $b=\gamma_2(c^{\prime}_1)$,
and $c_1 \leq c^{\prime}_1$. 
Note that $c_1 \leq c^{\prime}_1 \leq c$.
%%%
\begin{figure}[h]
\begin{tikzpicture}
\draw(0,0.5)--++(2,0.5)--++(0,-2)--++(-2,0.5)--cycle;
\draw(-3,0)--++(3,0.5);
\draw(-3,0)--++(3,-0.5);
\draw(-3,0)node[left]{$\gamma_1(0)$};
\draw(0,0.5)node[above]{$p_1$};
\draw(0,-0.5)node[below]{$p_2$};
\fill(-3,0)circle(0.06);
\draw(2,1)--++(1,1.5);
\draw(2,1)node[above]{$a$};
\draw(3,2.5)node[above]{$\gamma_1(1)$};
\fill(3,2.5)circle(0.06);
\draw(2,-1)--++(1,-1.5);
\draw(2,-1)node[right]{$b$};
%\draw(2.5,-1.75)node[right]{$\gamma_2(c)$};
\fill(2.5,-1.75)circle(0.06);;
\draw(3,-2.5)node[below]{$\gamma_2(1)$};
\fill(3,-2.5)circle(0.06);
%%%
\draw(2.5,1.5)node[right]{$\gamma_1(c)$};
\fill(2.5,1.75)circle(0.06);
\draw(3,-1.5)node{$\gamma_2(c)$};
\fill(2.5,-1.75)circle(0.06);
\end{tikzpicture}
\caption{Case IV)}
\label{eIII)}
\end{figure}
%%%
%\vspace{0.5cm}
%%%
Then, by Inequality \eqref{key3}, we have
\begin{align*}
&d(\gamma_1(c),\gamma_2(c))  \\
&=d(\gamma_1(c),a) + d(a,b) + d(b, \gamma_2(c)) \\
&=d(\gamma_1(c),\gamma_1(c_1)) + d(a,b)+ d(\gamma_2(c^{\prime}_1),\gamma_2(c)) \\
&=c\left(1-\dfrac{c_1}{c} \right)t + c^{\prime}_1d(\gamma_1(1),\gamma_2(1)) + c\left( 1-\dfrac{c^{\prime}_1}{c} \right)s \\
&\leq c(1-c_1)t + cd(\gamma_1(1),\gamma_2(1))+ c(1-c^{\prime}_1)s \\
&= c \{ d(\gamma_1(1),a) + d(b,\gamma_2(1)) \} + cd(\gamma_1(1),\gamma_2(1)) \\
&\leq c \{2 d(\gamma_1(1),\gamma_2(1)) \}.
\end{align*}

\par 
We consider case IV).
In case IV), we supposed that $\gamma_1(0)$, $\gamma_1(c)$, and $\gamma_2(c)$ are on the same geodesic segment.
Then we have that
\begin{align*}
d(\gamma_1(c),\gamma_2(c))&=c|t-s|\\
&\leq c d(\gamma_1(1),\gamma_2(1)).
\end{align*}
\par
Therefore, in case (\ref{ecase1})
we have 
%for all $\gamma_1, \gamma_2 \in \mathcal{L}_{\mathsf{Z}}$ with $\gamma_1(0)=\gamma_2(0)$,
\begin{equation}\label{cdiff}
d(\gamma_1(c), \gamma_2(c)) \leq c(2+E) d(\gamma_1(1),\gamma_2(1)) + ED + 4D +C.
\end{equation}
For $t,s,c \in [0,1]$, let $d_1=\gamma_1(t)$ and $d_2=\gamma_2(s)$
and let $\gamma'_1=\hat{\Gamma}(v,d_1)$ and $\gamma'_2=\hat{\Gamma}(v,d_2)$. 
By Lemma 3.3 and Inequality \ref{cdiff},  we have
%holds for all $c \in [0,1]$.
%Since $\gamma^{\prime}_1$, $\Gamma^{\prime}_2 \in \mathcal{L}_{\mathsf{Z}}$ with $\gamma^{\prime}_1 :[0,1] \to \mathsf{Z}$ and $\Gamma^{\prime}_2 : [0,1] \to \mathsf{Z}$, by \eqref{diff}, \eqref{1t}, and \eqref{2s},
\begin{align*}
&d(\gamma_1(ct), \gamma_2(cs)) \\
&\leq d(\gamma_1(ct),\gamma^{\prime}_1(c))+d(\gamma^{\prime}_1(c), \gamma^{\prime}_2(c)) +d(\gamma_2^{\prime}(c), \gamma_2(cs)) \\
& \leq c(2+E) d(\gamma^{\prime}_1(1),\gamma^{\prime}_2(1)) + ED + 4D + 3C \\
&=c(2+E) d(\gamma_1(t),\gamma_2(s))+ED + 4D +3C.
\end{align*}
Therefore, $\hat{\Gamma}$ satisfies assumption (\ref{gccc1}) of Lemma \ref{gccc}.
By the similar argument in proof of (\ref{TS-main-gcc}) of Theorem \ref{TS-Main_thm}, we obtain that $\hat{\Gamma}$ satisfies the assumption (\ref{gccc2}) of Lemma \ref{gccc}.
\par 
We consider the case (\ref{ecase2}).
The geodesic triangle $[\gamma_1(0),\gamma_1(1)] \cup [\gamma_1(1),\gamma_2(1)] \cup [\gamma_2(1),\gamma_1(0)]$ has the following form. %(see Figure \ref{gt}):
There exist $p_1, p_2 \in \psi(E(l_1))$ and $a, b \in \psi(E(l_2))$ such that
\begin{gather*}
[\gamma_1(0), \gamma_1(1)]= [\gamma_1(0), p_1] \cup [p_1,a] \cup [a, \gamma_1(1)] \ \mathrm{and} \\
[\gamma_1(0), \gamma_2(1)]= [\gamma_1(0), p_2] \cup [p_2,b] \cup [b, \gamma_2(1)].
%d(\gamma_1(1), \gamma_2(1))= d(\gamma_1(1), a) + d(a,b) + d(b, \gamma_2(1)) 
\end{gather*}
holds.
Note that $a,b \in \psi(E(l_2))$.
Then we have $d(a,b)\leq D$. 
%It was proved that the assumption of lemma holds when $p_1=p_2$. 
%Then, we suppose that $p_1 \neq p_2$. 
We set 
\begin{align*}
p_1&\coloneqq\gamma_1(c_0), \\
p_2&=\gamma_2(c_0^{\prime}), \\
a&\coloneqq\gamma_1(c_1), \\
b&\coloneqq\gamma_2(c_1^{\prime}),
\end{align*}
where $c_0, c_1, c_0^{\prime}, c_1^{\prime} \in [0,1]$.
%%%
%\begin{figure}[h]
%\begin{tikzpicture}
%\draw(0,0)--++(6,0)--++(-1,-1.5)--++(-6,0)--cycle; 
%\draw(5,-1.5)node[below]{$CX_k$};
%\draw[dashed](1,-1)--++(-0.5,-0.5);
%\draw(0.5,-1.5)--++(-1.5,-1.5);
%\draw(-1,-3)node[below]{$\gamma_1(0)$};
%\fill(-1,-3)circle(0.06);
%\draw(1,-1)--++(2,0.75)--++(0.75,-0.75)--cycle;
%\draw(1,-1)node[below]{$p$};
%\draw(3.5,-0.25)node[left]{$a$};
%\draw(3.75,-1)node[below]{$b$};
%\draw(3,-0.25)--++(1,2);
%\draw(4,1.75)node[above]{$\gamma_1(1)$};
%\fill(4,1.75)circle(0.06);
%\draw(3.75,-1)--++(3,1);
%\draw(6.75,0)node[above]{$\gamma_2(1)$};
%\fill(6.75,0)circle(0.06);
%\end{tikzpicture}
%\caption{In case ii), an example of geodesic triangles of $\mathsf{Z}$.}
%\label{gt}
%\end{figure}
%%%%
Set $t=d(\gamma_1(0),\gamma_1(1))$ and $s=d(\gamma_2(0),\gamma_2(1))$.
Since $p_1, p_2 \in \psi(E(l_1))$, we have $|c_0t-c_0^{\prime}s| \leq 2D$.
Without loss of generality, we may assume that $c_1 \leq c_1^{\prime}$.
We will show that 
there exist $E_{*} \geq 1$ and $C_* \geq 0$ depending only on $E$ and $C$ such that
for all $c \in [0,1]$, 
\begin{align*} 
d(\gamma_1(c), \gamma_2(c)) \leq cE_*d(\gamma_1(1), \gamma_2(1))+C_*.
\end{align*}
We divide the proof into the following cases: 
\begin{enumerate}
\renewcommand{\labelenumi}{\Roman{enumi}).}
\item \label{citemI)} $\gamma_1(c) \in [p_1,a]$ and $\gamma_2(c) \in [p_2,b]$ %(see Figure \ref{I)}).
\item \label{citemII)}$\gamma_1(c) \in [p_1,a]$ and $\gamma_2(c) \in [b, \gamma_2(1)]$ %(see Figure \ref{II)}).
\item \label{citemIII)}$\gamma_1(c) \in [a, \gamma_1(1)]$ and $\gamma_2(c) \in [b, \gamma_2(1)]$ %(see Figure \ref{III)}).
\item $\gamma_1(c) \in \gamma_2([0,c])$, or $\gamma_2(c) \in \gamma_1([0,c])$.
\end{enumerate}
In case I), we can put
\begin{align*}
\gamma_1(c)&=\Gamma(p_1,a)\left( \dfrac{c-c_0}{c_1-c_0}\right), \\
\gamma_2(c)& =\Gamma(p_2,b)\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}\right).
\end{align*}
%%%
%\begin{figure}[h]
%\begin{tikzpicture}
%\draw(0,0)--++(2,1)--++(0,-2)--cycle;
%\draw(-2,0)--++(2,0);
%\draw(-2,0)node[left]{$\gamma_1(0)$};
%\draw(0,0)node[above]{$p$};
%\fill(-2,0)circle(0.06);
%\draw(2,1)--++(1,1.5);
%\draw(2,1)node[above]{$a$};
%\draw(3,2.5)node[above]{$\gamma_1(1)$};
%\fill(3,2.5)circle(0.06);
%\draw(2,-1)--++(1,-1.5);
%\draw(2,-1)node[right]{$b$};
%\draw(3,-2.5)node[below]{$\gamma_2(1)$};
%\fill(3,-2.5)circle(0.06);
%%%
%\draw(1,0.5)node[above]{$\gamma_1(c)$};
%\fill(1,0.5)circle(0.06);
%\draw(1,-1)node{$\gamma_2(c)$};
%\fill(1,-0.5)circle(0.06);
%\end{tikzpicture}
%\caption{Case I)}
%\label{I)}
%\end{figure}
%%%
%Set $T\coloneqq(c_1-c_0)t$ and $S\coloneqq(c_1^{\prime}-c_0^{\prime})s$.
%Then we have
Note that
\begin{align*}
p_1&=\Gamma(p_1,a)(0), & p_2 &=\Gamma(p_2,b)\left( 0 \right), \\
\gamma_1(c)&=\Gamma(p_1,a)\left( \dfrac{c-c_0}{c_1-c_0}\right),                                     & a &=\Gamma(p_1,a)\left(1\right), \\ 
\gamma_2(c)&=\Gamma(p_2,b)\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}\right), & b &=\Gamma(p_2,b)\left(1\right).
\end{align*}
We define $a^{\prime} \in [p_1,a]$ to be
\begin{align*} 
a^{\prime}\coloneqq \Gamma(p_1,a)\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}\right).
\end{align*}
First, since $\Gamma$ is a geodesic $(E,C)$-coarsely convex bicombing, by the inequality $d(a,b) \leq D$, we have
\begin{align}
d(a^{\prime}, \gamma_2(c)) 
&=d \left( \Gamma(p_1,a)\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}\right) , \Gamma(p_2,b)\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}\right) \right)  \notag \\
&\leq \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} \cdot Ed(\Gamma(p_1,a)(1), \Gamma(p_2,b)(1)) \notag \\
&\ + \left( 1- \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} \right) \cdot Ed(\Gamma(p_1,a)(0), \Gamma(p_2,b)(0)) +C\notag \\
&= \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} \cdot Ed(a, b) +\left( 1- \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} \right)Ed(p_1,p_2) +C\notag \\
&\leq \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} \cdot ED +\left( 1- \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} \right)ED +C\notag \\
&\leq 2ED +C. \label{211}
\end{align}
Next, we consider the distance between $a^{\prime}$ and $\gamma_1(c)$.
Then
\begin{align*}
d(a^{\prime}, \gamma_1(c)) 
&=d \left( \Gamma(p_1,a)\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}\right) , \Gamma(p_1,a)\left( \dfrac{c-c_0}{c_1-c_0}\right) \right)  \notag \\
&=\left| \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} -\dfrac{c-c_0}{c_1-c_0}\right| \cdot d(p_1,a) \notag \\
&=\left| \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} -\dfrac{c-c_0}{c_1-c_0}\right| \cdot (c_1-c_0)t. \notag 
\end{align*}
By the triangle inequality $ (c_1-c_0)t  \leq (c_1^{\prime}-c_0^{\prime})s+ d(a,b)+ d(p_1,p_2)$, and $|c_0t-c_0's| \leq 2D$, we have
\begin{align*}
\left( \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} -\dfrac{c-c_0}{c_1-c_0} \right)(c_1-c_0)t 
&=\dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} (c_1-c_0)t  -\dfrac{c-c_0}{c_1-c_0}(c_1-c_0)t   \\
&\leq \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}  \{ (c_1^{\prime}-c_0^{\prime})s+ d(a,b) +d(p_1,p_2)\} -(c-c_0)t   \\
&\leq (c-c_0^{\prime})s -(c-c_0)t +\dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} d(a,b) +\dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} d(p_1,p_2)\\
&\leq c(s-t) + (c_0t-c_0^{\prime}s) + 2D \\
&\leq c d(\gamma_1(1), \gamma_2(1)) +4D.
\end{align*}
Similarly, by the triangle inequality $ (c_1^{\prime}-c_0^{\prime})s - d(a,b)-d(p_1,p_2)  \leq  (c_1-c_0)t$, and $|c_0t-c_0's| \leq 2D$, we have
\begin{align*}
\left( \dfrac{c-c_0}{c_1-c_0} - \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} \right) (c_1-c_0)t 
&=\dfrac{c-c_0}{c_1-c_0}(c_1-c_0)t  - \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} (c_1-c_0)t  \\
&\leq (c-c_0)t -\dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}  \{ (c_1^{\prime}-c_0^{\prime})s - d(a,b)-d(p_1,p_2)\} \\
&= (c-c_0)t - (c-c_0^{\prime})s +\dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} d(a,b) +\dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}}d(p_1,p_2) \\
&\leq c(t-s) + (c_0's-c_0t) + 2D\\
&\leq c d(\gamma_1(1), \gamma_2(1))+4D.
\end{align*}
Then we have
\begin{align}
d(a^{\prime}, \gamma_1(c))
&=\left| \dfrac{c-c_0^{\prime}}{c_1^{\prime}-c_0^{\prime}} -\dfrac{c-c_0}{c_1-c_0}\right| \cdot (c_1-c_0)t \notag \\
&\leq c d(\gamma_1(1), \gamma_2(1)) +4D. \label{212}
\end{align}
Combining \eqref{211} and \eqref{212} yields
\begin{align*}
d(\gamma_1(c),\gamma_2(c)) 
&\leq d(\gamma_1(c),a^{\prime}) + d(a^{\prime}, \gamma_2(c)) \\ 
& \leq c d(\gamma_1(1), \gamma_2(1)) + 2ED +4D +C \\
& = c d(\gamma_1(1), \gamma_2(1)) +2ED +4D +C.
\end{align*}
%By a similar argument, 
\textcolor{red}{We can omit.}
\end{comment}
%%%

\begin{comment}
We consider case iii), case iv), and case vi).
By the same argument in case ii), we have
\begin{align*}
d(\gamma_1(c),\gamma_2(c)) \leq c d(\gamma_1(1), \gamma_2(1)) +2ED +4D +C.
\end{align*}
\par 
By the similar argument in the proof of (\ref{TS-main-gcc}) of Theorem \ref{TS-Main_thm}, 
%in case (\ref{ecase2}), 
we obtain that $\hat{\Gamma}_k$ satisfies the assumption (\ref{ccgccc2}) of Lemma \ref{ccgccc}.
Therefore, by Lemma \ref{ccgccc}, we show that $\hat{\Gamma}$ is a geodesic coarsely convex bicombing. 
\end{comment}





==> 70-Examples.tex <==
In this section, we provide examples of relatively geodesic coarsely convex groups.
First, we give examples of geodesic coarsely convex spaces and groups.
\subsection{Geodesic coarsely convex spaces and groups}
The following metric spaces admit geodesic coarsely convex bicombings.
\begin{enumerate}
 \item geodesic Gromov hyperbolic spaces
 \item CAT(0) spaces
 \item Busemann spaces
 \item systolic complexes~\cite{bdrySytolic}
 \item proper injective metric spaces~\cite{convex-bicomb}
 \item Helly graphs~\cite{chalopin2020helly-arXiv}
\end{enumerate}

We remark that in the above list, all geodesic bicombings are invariant under isometries. 
We say that a group is systolic if it acts properly and cocompactly on a systolic complex
by simplicial automorphisms.
\begin{theorem}[Osajda-Huang, Osajda-Prytu{\l}a]
  Artin groups of large type~\cite{MR3999678} and 
   graphical $C(6)$ small cancellation groups~\cite{MR3845715} are systolic.
\end{theorem}

We say that a group is Helly if it acts properly and cocompactly 
on a Helly graph by graph automorphisms. 
\begin{theorem}[Osajda-Huang]
Weak Garside groups of finite type and Artin groups of type FC 
are Helly~\cite{MR4285138}.
\end{theorem}

For concrete examples of Garside groups, see the introduction of \cite{MR4285138}.

\subsection{Relatively geodesic coarsely convex groups}

%\begin{itemize}
%\item
%\taku{complex of groups} 
%\item
%\taku{\cite[Example 8.4]{zbMATH06941810}}
%\item
%\taku{We define relatively coarsely convexity based on Gromov's def of rel hyp.
%(a generalization of geometric finite action) }
%\item
%\taku{``Automorphisms and outer automorphisms groups of Right-angled Artin groups are not relatively hyperbolic'' \cite{KIM}}
%\item
%\taku{cofinte actions of lattices of higher rank symmetric spaces suggested by Kondo}
%\item 
%\taku{Relatively CAT(0), relatively systolic.}
%\item 
%\taku{
%In a coarsely convex space, coning off quasi-convex subspaces, does the resulting space remain coarsely convex?
%}
%\item 
%\subsubsection{}
Let $F_2 = \langle a, b \rangle$ be the free group of rank $2$
and let $S=\{a,b\}$ be the standard generating set. 
For a subgroup $A= \langle a \rangle$, 
we consider the coned-off Cayley graph $\hat{\Gamma}(F_2\times \mathbb{Z},A,S)$ as a metric graph. 
It is easily shown that $\mathbb{Z} \times \mathbb{Z}$ can be quasi-isometrically embedded on $\hat{\Gamma}(F_2\times \mathbb{Z},A,S)$.
Then $(F_2 \times \mathbb{Z},A)$ is not a relatively hyperbolic group. 
In \cite{Tp}, it is shown that $\hat{\Gamma}(F_2\times \mathbb{Z},A,S)$ admit a geodesic coarsely convex bicombing. 
Therefore, $(F_2 \times \mathbb{Z}, A)$ is a relatively geodesic coarsely convex groups. 
%Certainly, it is geodesic coarsely convex. 
%\item 
%$(\mathbb{Z}^3 \ast \mathbb{Z}^2, \mathbb{Z}^3)?$
%\end{itemize}


==> 80-BoundedCosetPenetration.tex <==
In this section, we define strong relatively geodesic coarsely convex groups.

\subsection{Strong relatively hyperbolic spaces}

In \cite{PK}, Abhijit Pal and Akshay Kumar Singh gave two definition of relatively hyperbolic spaces based on the notions of relatively hyperbolic groups given by Gromov and Farb.

Among their definitions, we will review the one based on Farb’s approach.
Let $(X, d)$ be a path metric space. 
Let $\mathcal{H}$ be a collection of closed and path connected subsets $\{H\alpha \}_{\alpha \in \Lambda}$ of $X$ 
such that each $H\alpha$ is a intrinsically geodesic space with the induced path metric, denoted by $d_{H\alpha}$. 
For $\nu > 1$, the collection $H$ are uniformly $\nu$-separated.
%The elements of H are said to be uniformly properly embedded in $X$ 
%if for all $M > 0$ there exists $N(M) > 0$ such that for all $H \alpha \in \amthcal{H}$
%and for all $x, y \in H \alpha$ if $d(x, y) \geq M$ then $d_{H \alpha} (x, y) \geq N$.

Let $E(X,\mathcal{H})$ be the quotient space of $X \bigsqcup (\sqcup_{\alpha} (H_{\alpha} \times [0, 1/2]))$ 
obtained by identifying each $H_{\alpha} \times \{1/2\}$ to a point $v(H_{\alpha})$ 
and for all $h \in H\alpha$, $(h, 0)$ is identified with $h$. 
Let $d_E$ be the quotient metric on $E(X, \mathcal{H})$.
The space $\hat{X}$ constructed above corresponding to the pair $(X, \mathcal{H})$ is said to be electric space.

\begin{definition}
\begin{itemize}
\item[]
\item 
A path $\gamma \in \hat{X}$ is said to be an electric geodesic (resp. electric $(K,K)$-quasigeodesic) 
if it is a geodesic (resp. $(K,K)$-quasigeodesic) in $\hat{X}$.

\item 
For a path $\gamma$ on $X$, there is a path $\hat{\gamma}$ in $\hat{X}$ obtained from $\gamma$ as follows: 
if $\gamma$ penetrates a horosphere-like set $H$ with entry point $x$ and exit point $y$, we replace
the portion of the path $\gamma$ lying inside $H$ joining $x$, $y$ by $[x, v(H)] \cup [v(H) , y]$, 
where $v(H)$ is the cone point over $H$, $[x, v(H)]$ and $[v(H) , y]$ are electric geodesic segments of
length 1/2 joining $x, v(H)$ and $v(H) , y$ respectively. 

If $\hat{\gamma}$ is an electric geodesic (resp. $(P,P)$-quasigeodesic), 
$\gamma$ is called a relative geodesic (resp. relative $(P,P)$-quasigeodesic).
\end{itemize}
\end{definition}

\begin{definition}
Relative geodesics (resp. $(P,P)$-quasigeodesic paths) in $E(X, H)$ are said to satisfy \emph{bounded horosphere penetration}
if for any two relative geodesics (resp. $(P,P)$-quasigeodesic paths without backtracking) $\beta$, $\gamma$, joining $x, y \in X$ there exists $C > 0$ such that

\begin{itemize}
    \item
    \emph{Similar Intersection Patterns 1}: 
    if precisely one of $\{\beta, \gamma\}$ meets a horosphere-like set $H_{\alpha}$, then the distance (measured in the intrinsic path-metric on $H_{\alpha}$) from the entry point to the exit point (of the relevant path) is at most $C$.

    \item
    \emph{Similar Intersection Patterns 2}: 
    if both $\{\beta, \gamma\}$ meet some $H_{\alpha}$ then the distance (measured in the intrinsic path-metric on $H_{\alpha}$) from the entry point of $\beta$ to that of $\gamma$ is at most $C$; similarly for exit points.
\end{itemize}
\end{definition}

\begin{definition}
Let $\delta \geq 0$. 
Let $X$ be a geodesic metric space and
$\mathcal{H}$ be a collection of uniformly $\nu$-separated and 
intrinsically geodesic closed subsets of $X$. 
Then $X$ is said to be $\delta$-hyperbolic relative to the collection H in the sense of Farb if
\begin{enumerate}
    \item $E(X,\mathcal{H})$ is hyperbolic,
    \item Relative $(P,P)$-quasigeodesic paths without backtracking satisfy the bounded horosphere penetration properties.
\end{enumerate}
\end{definition}

\subsection{Strong relatively geodesic coarsely convex groups}

\begin{definition}
\begin{enumerate}
  \item[]
  \item 
  A group pair $(G,\mathcal{H})$ is a \emph{strong coarsely convex} if there is a Cayley--Abels graph which admits a coarsely convex bicombing and satisfies bounded coset penetration.

  \item 
  A group pair $(G,\mathcal{H})$ is \emph{strong geodesic coarsely convex} 
  if $G$ acts cocompactly and by isometries on a geodesic coarsely convex metric space $X$ such that 
  \begin{enumerate}
  \item
 for every $H\in\mathcal{H}$ the fixed point set $X^H$ is non-empty and bounded; 
 \item 
 and for each $x\in X$ the isotropy $G_x$ is either finite or conjugate to some $H\in\mathcal{H}$.
 \item 
 and $X$ satisfies bounded horosphere condition.
 \end{enumerate}
\end{enumerate}


\end{definition}

%Let $e$ be a edge in tree $T$ whose one of the endpoints is in $L$. 
%We say a preimage $\xi^{-1}(e)$ a \emph{horosphere-like set}

\begin{conjecture}
Let $Z$ be a tree of spaces associated with a map $\xi\colon Z\to T$, where $V(T)=K \sqcup L$. 
Suppose that each $X_k=\xi^{-1}(\starNb(k))$ admits a bicombing ${\Gamma}_k \colon X_k \times X_k \times [0,1] \to X_k$.
There is a bicombing $\Gamma \colon Z  \times Z \times [0,1] \to Z$ on $Z$ satisfying the following properties.
\begin{enumerate}
    \item Each $X_k$ satisfies BHP property, then $Z$ satisfies BHP property.
\end{enumerate}
\end{conjecture}


